Adjoint Complement to the Volume-of-Fluid Method for Immiscible Flows

The paper is concerned with an adjoint complement to the Volume-of-Fluid (VoF) method for immiscible two-phase flows, e.g. air and water, which is widely used in marine engineering due to its computational efficiency. The particular challenge of the primal and the corresponding adjoint VoF-approach refers to the sharp interface treatment featuring discontinuous physical properties. Both the continuous adjoint two-phase system (integration-by-parts) and the corresponding dual compressive convection schemes (summation-by-parts) are derived for two prominent compressive convection schemes, namely the High Resolution Interface Capturing Scheme (HRIC) and Compressive Interface Capturing Scheme for Arbitrary Meshes (CICSAM). The dual scheme rigorously mirrors the primal Normalized-Variable-Diagram (NVD) stencils. Attention is restricted to steady state applications. Thus both the primal and the dual procedures are performed in pseudo time and the backward integration of the dual approach is performed around the (pseudo-temporal) converged primal field. The paper analyses the primal and adjoint equations for an engineering model problem. An analytical solution to the model problem is initially presented, which displays that the adjoint part does not offer a unique, non-trivial solution. As a remedy, an additional diffusive concentration term is introduced to the adjoint concentration equation. Numerical results obtained from the modified approach are benchmarked against the analytical solution for the model problem. Supplementary, the influence of the modification on the sensitivities obtained from simulations for the two-dimensional flow around a submerged hydrofoil are discussed. The final application refers to a shape-optimization of a generic 3D underwater vehicle and underlines a negligible influence of the free mobility parameter.

==> tex/derivation_area.tex <==
\section{Derivation Area}

\subsection{Differentiation Through the Interface Orientation}
Several 'if-else' like statements arise within the compressive VoF schemes which can be relatively easy inverted w.r.t. dual consistency. However, one crucial interceptor accounts for the free-surface to velocity alignment $\mathrm{cos}(\theta^\mathrm{F})$, where the angle is usually implemented based on the local grid arrangement, viz.
\begin{align}
\theta^\mathrm{F} \approx \frac{\frac{\partial c}{\partial x_\mathrm{i}} \Delta x_\mathrm{i}}{||\frac{\partial c}{\partial x_\mathrm{i}} || || \Delta x_\mathrm{i}||}.
\end{align}
The continuous interpretation should read somehow
\begin{align}
\theta = || \frac{\partial c}{\partial x_\mathrm{i}} v_\mathrm{i} ||
\end{align}
Remembering the implementation of the compressive schemes yields an face value estimation of approximately:
\begin{align}
\int_\mathrm{\Omega^*} \hat{c}^* v_\mathrm{k}^* \frac{\partial c}{\partial x_\mathrm{k}^*} \mathrm{d} \Omega^* &= \int_\mathrm{\Gamma^*} \hat{c}^* v_\mathrm{k}^* n_\mathrm{k} \mathrm{d} \Gamma^* - \int_\mathrm{\Omega^*} c v_\mathrm{k}^* \frac{\partial \hat{c}^*}{\partial x_\mathrm{k}^*} \mathrm{d} \Omega^*
\end{align}
or in discrete space
\begin{align}
\sum_\mathrm{P} \left[ \hat{c} v_\mathrm{k} \frac{\partial c}{\partial x_\mathrm{k}}  \right]^\mathrm{*P} &= \sum_\mathrm{P} \hat{c}^\mathrm{*P} \sum_\mathrm{F(P)} \bigg[ \dot{V}^* c \bigg]^\mathrm{F} \\
&\approx ... + \hat{c}^\mathrm{*P} \sum_\mathrm{F(P)}  \left[ \mathrm{cos} \left(|| \frac{\partial c}{\partial x_\mathrm{i}}^* v_\mathrm{i}^* ||\right) \dot{V}^{*F+} c^{F+} + \left(1 - \mathrm{cos} \left(|| \frac{\partial c}{\partial x_\mathrm{i}}^* v_\mathrm{i}^* ||\right) \dot{V}^{*F-} c^{F-} \right) \right] + ...
\end{align}
where the superscripts +/- account for the positive/negative free-surface side. Obviously, a derivative in concentration direction needs 1) the inverse cosine operator and 2) a subsequent integration by parts. Such a nested relation seems to be similar to TVD limiters within classical, non-compressive CFD and is therefore skipped during the backward simulation.

\subsection{Diffusion from Momentum Equation}
The discrete diffusive (Laplacian) operator can be evaluated as follows:
\begin{alignat*}{10}
 \sum_\mathrm{P} \hat{v}_\mathrm{i}^\mathrm{*P} \sum_\mathrm{F(P)} \bigg[ 2 \mu^* S_\mathrm{ik}^* \Delta \Gamma_\mathrm{k}^* \bigg]^\mathrm{F} = ... 
 &+ 2 \hat{v}_\mathrm{i}^\mathrm{*UU} &&\bigg[ \frac{1}{2} \bigg( \mu^\mathrm{*U}&&-\mu^\mathrm{*UU} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*U} &&-S_\mathrm{ik}^\mathrm{*UU}\bigg) 
 &&-  \frac{1}{2} \bigg( \mu^\mathrm{*UU} &&-\mu^\mathrm{*UUU}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*UU} && -S_\mathrm{ik}^\mathrm{*UUU}   \bigg) &&\bigg] \\
&+ 2 \hat{v}_\mathrm{i}^\mathrm{*U} &&\bigg[ \frac{1}{2} \bigg( \mu^\mathrm{*D}&&-\mu^\mathrm{*U} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*D} &&-S_\mathrm{ik}^\mathrm{*U}\bigg) 
 &&-  \frac{1}{2} \bigg( \mu^\mathrm{*U} &&-\mu^\mathrm{*UU}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*U} && -S_\mathrm{ik}^\mathrm{*UU}   \bigg) &&\bigg] \\
&+ 2 \hat{v}_\mathrm{i}^\mathrm{*D} &&\bigg[ \frac{1}{2} \bigg( \mu^\mathrm{*DD}&&-\mu^\mathrm{*D} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*DD} &&-S_\mathrm{ik}^\mathrm{*D}\bigg) 
 &&-  \frac{1}{2} \bigg( \mu^\mathrm{*D} &&-\mu^\mathrm{*U}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*D} && -S_\mathrm{ik}^\mathrm{*U}   \bigg) &&\bigg] \\
&+ 2 \hat{v}_\mathrm{i}^\mathrm{*DD} &&\bigg[ \frac{1}{2} \bigg( \mu^\mathrm{*DDD}&&-\mu^\mathrm{*DD} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*DDD} &&-S_\mathrm{ik}^\mathrm{*DD}\bigg) 
 &&-  \frac{1}{2} \bigg( \mu^\mathrm{*DD} &&-\mu^\mathrm{*D}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*DD} && -S_\mathrm{ik}^\mathrm{*D}   \bigg) &&\bigg].
\end{alignat*}
A variation in $c$ yields:
\begin{alignat*}{10}
\delta_\mathrm{c} \tilde{L}^*  \cdot \delta c ... = ... 
 &+ 2 \hat{v}_\mathrm{i}^\mathrm{*UU} \mu_\Delta &&\bigg[ \frac{1}{2} \bigg( \delta_c^\mathrm{*U}&&-\delta_c^\mathrm{*UU} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*U} &&-S_\mathrm{ik}^\mathrm{*UU}\bigg) 
 &&-  \frac{1}{2} \bigg( \delta_c^\mathrm{*UU} &&-\delta_c^\mathrm{*UUU}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*UU} && -S_\mathrm{ik}^\mathrm{*UUU}   \bigg) &&\bigg] \\
&+ 2 \hat{v}_\mathrm{i}^\mathrm{*U} \mu_\Delta &&\bigg[ \frac{1}{2} \bigg( \delta_c^\mathrm{*D}&&-\delta_c^\mathrm{*U} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*D} &&-S_\mathrm{ik}^\mathrm{*U}\bigg) 
 &&-  \frac{1}{2} \bigg( \delta_c^\mathrm{*U} &&-\delta_c^\mathrm{*UU}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*U} && -S_\mathrm{ik}^\mathrm{*UU}   \bigg) &&\bigg] \\
&+ 2 \hat{v}_\mathrm{i}^\mathrm{*D} \mu_\Delta&&\bigg[ \frac{1}{2} \bigg( \delta_c^\mathrm{*DD}&&-\delta_c^\mathrm{*D} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*DD} &&-S_\mathrm{ik}^\mathrm{*D}\bigg) 
 &&-  \frac{1}{2} \bigg( \delta_c^\mathrm{*D} &&-\delta_c^\mathrm{*U}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*D} && -S_\mathrm{ik}^\mathrm{*U}   \bigg) &&\bigg] \\
&+ 2 \hat{v}_\mathrm{i}^\mathrm{*DD} \mu_\Delta &&\bigg[ \frac{1}{2} \bigg( \delta_c^\mathrm{*DDD}&&-\delta_c^\mathrm{*DD} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*DDD} &&-S_\mathrm{ik}^\mathrm{*DD}\bigg) 
 &&-  \frac{1}{2} \bigg( \delta_c^\mathrm{*DD} &&-\delta_c^\mathrm{*D}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*DD} && -S_\mathrm{ik}^\mathrm{*D}   \bigg) &&\bigg].
\end{alignat*}
that can be rearranged to:
\begin{alignat*}{10}
\delta_\mathrm{c} \tilde{L}^*  \cdot \delta c ... = ... 
 &+ 2 \delta_c^\mathrm{*UU} \mu_\Delta &&\bigg[ \frac{1}{2} \bigg( \hat{v}_\mathrm{i}^\mathrm{*U}&&-\hat{v}_\mathrm{i}^\mathrm{*UU} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*U} &&-S_\mathrm{ik}^\mathrm{*UU}\bigg) 
 &&-  \frac{1}{2} \bigg( \hat{v}_\mathrm{i}^\mathrm{*UU} &&-\hat{v}_\mathrm{i}^\mathrm{*UUU}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*UU} && -S_\mathrm{ik}^\mathrm{*UUU}   \bigg) &&\bigg] \\
&+ 2 \delta_c^\mathrm{*U} \mu_\Delta &&\bigg[ \frac{1}{2} \bigg( \hat{v}_\mathrm{i}^\mathrm{*D}&&-\hat{v}_\mathrm{i}^\mathrm{*U} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*D} &&-S_\mathrm{ik}^\mathrm{*U}\bigg) 
 &&-  \frac{1}{2} \bigg( \hat{v}_\mathrm{i}^\mathrm{*U} &&-\hat{v}_\mathrm{i}^\mathrm{*UU}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*U} && -S_\mathrm{ik}^\mathrm{*UU}   \bigg) &&\bigg] \\
&+ 2 \delta_c^\mathrm{*D} \mu_\Delta&&\bigg[ \frac{1}{2} \bigg( \hat{v}_\mathrm{i}^\mathrm{*DD}&&-\hat{v}_\mathrm{i}^\mathrm{*D} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*DD} &&-S_\mathrm{ik}^\mathrm{*D}\bigg) 
 &&-  \frac{1}{2} \bigg( \hat{v}_\mathrm{i}^\mathrm{*D} &&-\hat{v}_\mathrm{i}^\mathrm{*U}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*D} && -S_\mathrm{ik}^\mathrm{*U}   \bigg) &&\bigg] \\
&+ 2 \delta_c^\mathrm{*DD} \mu_\Delta &&\bigg[ \frac{1}{2} \bigg( \hat{v}_\mathrm{i}^\mathrm{*DDD}&&-\hat{v}_\mathrm{i}^\mathrm{*DD} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*DDD} &&-S_\mathrm{ik}^\mathrm{*DD}\bigg) 
 &&-  \frac{1}{2} \bigg( \hat{v}_\mathrm{i}^\mathrm{*DD} &&-\hat{v}_\mathrm{i}^\mathrm{*D}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*DD} && -S_\mathrm{ik}^\mathrm{*D}   \bigg) &&\bigg]
\end{alignat*}
where a switch in sign can be realized:
\begin{alignat*}{10}
\delta_\mathrm{c} \tilde{L}^*  \cdot \delta c ... = ... 
 &- 2 \delta_c^\mathrm{*UU} \mu_\Delta &&\bigg[ \frac{1}{2} \bigg( -\hat{v}_\mathrm{i}^\mathrm{*U}&&+\hat{v}_\mathrm{i}^\mathrm{*UU} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*U} &&-S_\mathrm{ik}^\mathrm{*UU}\bigg) 
 &&-  \frac{1}{2} \bigg( -\hat{v}_\mathrm{i}^\mathrm{*UU} &&+\hat{v}_\mathrm{i}^\mathrm{*UUU}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*UU} && -S_\mathrm{ik}^\mathrm{*UUU}   \bigg) &&\bigg] \\
&- 2 \delta_c^\mathrm{*U} \mu_\Delta &&\bigg[ \frac{1}{2} \bigg( -\hat{v}_\mathrm{i}^\mathrm{*D}&&+\hat{v}_\mathrm{i}^\mathrm{*U} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*D} &&-S_\mathrm{ik}^\mathrm{*U}\bigg) 
 &&-  \frac{1}{2} \bigg( -\hat{v}_\mathrm{i}^\mathrm{*U} &&+\hat{v}_\mathrm{i}^\mathrm{*UU}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*U} && -S_\mathrm{ik}^\mathrm{*UU}   \bigg) &&\bigg] \\
&- 2 \delta_c^\mathrm{*D} \mu_\Delta&&\bigg[ \frac{1}{2} \bigg( -\hat{v}_\mathrm{i}^\mathrm{*DD}&&+\hat{v}_\mathrm{i}^\mathrm{*D} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*DD} &&-S_\mathrm{ik}^\mathrm{*D}\bigg) 
 &&-  \frac{1}{2} \bigg( -\hat{v}_\mathrm{i}^\mathrm{*D} &&+\hat{v}_\mathrm{i}^\mathrm{*U}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*D} && -S_\mathrm{ik}^\mathrm{*U}   \bigg) &&\bigg] \\
&- 2 \delta_c^\mathrm{*DD} \mu_\Delta &&\bigg[ \frac{1}{2} \bigg( -\hat{v}_\mathrm{i}^\mathrm{*DDD}&&+\hat{v}_\mathrm{i}^\mathrm{*DD} \bigg)  &&\frac{1}{2} \bigg(  S_\mathrm{ik}^\mathrm{*DDD} &&-S_\mathrm{ik}^\mathrm{*DD}\bigg) 
 &&-  \frac{1}{2} \bigg( -\hat{v}_\mathrm{i}^\mathrm{*DD} &&+\hat{v}_\mathrm{i}^\mathrm{*D}\bigg)  &&\frac{1}{2} \bigg( S_\mathrm{ik}^\mathrm{*DD} && -S_\mathrm{ik}^\mathrm{*D}   \bigg) &&\bigg]
\end{alignat*}

\subsection{Implementation Details}

The following field are used for the generic implementation of different convection schemes:
\begin{alignat}{3}
\mathrm{As}^\mathrm{F}(s_\mathrm{1}) &\rightarrow \mathrm{As}(s_\mathrm{1}) + \mathrm{min}(\dot{V},0) \qquad &&\mathrm{As}^\mathrm{F}(s_\mathrm{2}) &&\rightarrow \mathrm{As}(s_\mathrm{2}) - \mathrm{max}(\dot{V},0) \\
\mathrm{Dc}^\mathrm{F} &\rightarrow \mathrm{Dc}^\mathrm{F} - \mathrm{min}(\dot{V},0) \phi^\mathrm{C}(s2) - \mathrm{max}(\dot{V},0) \phi^\mathrm{C}(s1) + \dot{V} \, \mathrm{HOC} \\
\mathrm{S}^\mathrm{C}(s_\mathrm{1}) &\rightarrow \mathrm{S}(s_\mathrm{1}) - \mathrm{Dc}^\mathrm{F} \qquad &&\mathrm{S}^\mathrm{C}(s_\mathrm{2}) &&\rightarrow \mathrm{S}(s_\mathrm{2}) + \mathrm{Dc}^\mathrm{F} \\
\mathrm{A}^\mathrm{C}(s_\mathrm{1}) &\rightarrow \mathrm{A}(s_\mathrm{1}) - \mathrm{As}^\mathrm{F}(s_\mathrm{1}) \qquad &&\mathrm{A}^\mathrm{C}(s_\mathrm{2}) &&\rightarrow \mathrm{A}(s_\mathrm{2}) - \mathrm{As}^\mathrm{F}(s_\mathrm{2})
\end{alignat}
where $\mathrm{As}^\mathrm{F}$, $\mathrm{Dc}^\mathrm{F}$, $\mathrm{S}^\mathrm{C}$ and $\mathrm{A}^\mathrm{C}$ represent the neighbour cells of a face, the deferred correction of each internal face, the source term as well as the main diagonal coefficient. HOC stands for High Order Convection. In general we end up with the following line within the discrete system:
\begin{align}
A^\mathrm{P} \phi^\mathrm{P} - \sum_{\mathrm{NB}} A^\mathrm{NB} \phi^\mathrm{NB} = S^\mathrm{P}.
\end{align}
Stability problems w.r.t. downwinding certain face values become clear for the cell Q in Fig \ref{fig:1d_flow_discretized}, viz.
\begin{align}
\left[ \frac{\Delta \Omega}{\Delta t} + \dot{V} \right] \phi^\mathrm{Q,t} + \dot{V} \phi^\mathrm{P,t}  = \phi^\mathrm{Q,t-1}\frac{\Delta \Omega}{\Delta t} + \dot{V} \left[ -\phi^\mathrm{P,t-1} + \phi^\mathrm{Q,t-1} + \phi^\mathrm{Q,t-1} - \phi^\mathrm{R,t-1} \right].
\end{align}
where we have approximated the temporal derivative with a first order forward Euler stencil. Assuming $\phi^{(\cdot),t-1} \approx \phi^\mathrm{(\cdot),t}$, reordering yields:
\begin{align}
\left[ \frac{\Delta \Omega}{\Delta t} - \dot{V} \right] \phi^\mathrm{Q,t} + 2 \dot{V} \phi^\mathrm{P,t} + \dot{V} \phi^\mathrm{R}  = \phi^\mathrm{Q,t-1}\frac{\Delta \Omega}{\Delta t}.
\end{align}
Multiplication with $\Delta \Omega / \Delta t$ offers a main diagonal coefficient of $A^\mathrm{Q} = 1 - \mathrm{Co}$ with $\mathrm{Co} = \dot{V} \Delta t / \Delta \Omega$. \nkuehl{Ich mache i.d.R. nur eine {\"a}ussere Iteration pro Zeitschritt, daher ist die rechte Seite zeitlich gesehen explizit, was schlussendlich die Annahme $\phi^{(\cdot),t-1} \approx \phi^\mathrm{(\cdot),t}$ rechtfertigt}

\begin{landscape}

\begin{figure}
\centering
\input{./tikz/1D_Flow_Discretized.tikz}
\caption{Schematic one dimensional view of the discretization for a primal/dual compressive (downwind biased) convection scheme to capture an interface between cell P and R (pure downwinding at PQ and QR).}
\label{fig:1d_flow_discretized}
\end{figure}

\end{landscape}

